Purifying Interaction Effects with the Functional ANOVA: An Efficient Algorithm for Recovering Identifiable Additive Models

Models which estimate main effects of individual variables alongside interaction effects have an identifiability challenge: effects can be freely moved between main effects and interaction effects without changing the model prediction. This is a critical problem for interpretability because it permits "contradictory" models to represent the same function. To solve this problem, we propose pure interaction effects: variance in the outcome which cannot be represented by any smaller subset of features. This definition has an equivalence with the Functional ANOVA decomposition. To compute this decomposition, we present a fast, exact algorithm that transforms any piecewise-constant function (such as a tree-based model) into a purified, canonical representation. We apply this algorithm to Generalized Additive Models with interactions trained on several datasets and show large disparity, including contradictions, between the effects before and after purification. These results underscore the need to specify data distributions and ensure identifiability before interpreting model parameters.

==> log_figure_intx.tex <==

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.4\columnwidth}
        \vskip 0pt
        \centering
        \includegraphics[width=\textwidth]{figs/log/log_intx_lam_0.pdf}
        \caption{Raw Interaction, $\lambda=0.0$}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.4\columnwidth}
        \vskip 0pt
        \centering
        \includegraphics[width=\textwidth]{figs/log/log_intx_pure_lam_0.pdf}
        \caption{Pure Interaction, $\lambda=0.0$}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.4\columnwidth}
        \vskip 0pt
        \centering
        \includegraphics[width=\textwidth]{figs/log/log_intx_lam_1000.pdf}
        \caption{Raw Interaction, $\lambda=1.0$}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.4\columnwidth}
        \vskip 0pt
        \centering
        \includegraphics[width=\textwidth]{figs/log/log_intx_pure_lam_1000.pdf}
        \caption{Pure Interaction, $\lambda=1.0$}
    \end{subfigure}
    \caption{Interaction effects in the log model \eqref{eq:log_model}. For $\lambda=0$, there is no pure interaction effect. For $\lambda=1$, there is pure interaction effect in the form of the continuous XOR.}
    \label{fig:log_interactions}
\end{figure}


==> log_figure_mains.tex <==

\begin{figure}[H]
    \centering
    \vskip 0pt
    \begin{subfigure}[t]{0.31\columnwidth}
        \vskip 0pt
        \centering
        \includegraphics[width=\textwidth]{figs/log/new/main_effect_x1_lam_0.pdf}
        \caption{$\lambda = 0.0$}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.31\columnwidth}
        \vskip 0pt
        \centering
        \includegraphics[width=\textwidth]{figs/log/new/main_effect_x1_lam_500.pdf}
        \caption{$\lambda = 0.5$}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.31\columnwidth}
        \vskip 0pt
        \centering
        \includegraphics[width=\textwidth]{figs/log/new/main_effect_x1_lam_1000.pdf}
        \caption{$\lambda = 1.0$}
    \end{subfigure}
    \caption{Pure Main Effects of the log model \eqref{eq:log_model}. The purification algorithm recovers the transition from logarithmic to linear main effects.}
    \label{fig:log_mains}
\end{figure}

